Extinction and dust/gas ratio in the H I ridge region of the LMC based on the IRSF/SIRIUS near-infrared survey

We present a dust extinction AV map of the Large Magellanic Cloud (LMC) in the H I ridge region using the IRSF near-infrared (IR) data, and compare the AV map with the total hydrogen column density N(H) maps derived from the CO and H I observations. In the LMC H I ridge region, the two-velocity H I components (plus an intermediate velocity component) are identified, and the young massive star cluster is possibly formed by collision between them. In addition, one of the components is suggested to be an inflow gas from the Small Magellanic Cloud (SMC) which is expected to have even lower metallicity gas (Fukui et al. 2017, PASJ, 69, L5). To evaluate dust/gas ratios in the H I ridge region in detail, we derive the AV map from the near-IR color excess of the IRSF data updated with the latest calibration, and fit the resultant AV map with a combination of the N(H) maps of the different velocity components to successfully decompose it into the 3 components. As a result, we find difference by a factor of 2 in AV /N(H) between the components. In additon, the CO-to-H2 conversion factor also indicates difference between the components, implying the difference in the metallicity. Our results are likely to support the scenario that the gas in the LMC H I ridge region is contaminated with an inflow gas from the SMC with a geometry consistent with the on-going collision between the two velocity components.

==> 00README.tex <==
nohypertex
